Automated tight Lyapunov analysis for first-order methods

We present a methodology for establishing the existence of quadratic Lyapunov inequalities for a wide range of first-order methods used to solve convex optimization problems. In particular, we consider i) classes of optimization problems of finite-sum form with (possibly strongly) convex and possibly smooth functional components, ii) first-order methods that can be written as a linear system in state-space form in feedback interconnection with the subdifferentials of the functional components of the objective function, and iii) quadratic Lyapunov inequalities that can be used to draw convergence conclusions. We present a necessary and sufficient condition for the existence of a quadratic Lyapunov inequality within a predefined class of Lyapunov inequalities, which amounts to solving a small-sized semidefinite program. We showcase our methodology on several first-order methods that fit the framework. Most notably, our methodology allows us to significantly extend the region of parameter choices that allow for duality-gap convergence in the Chambolle-Pock method when the linear operator is the identity mapping.

==> ChambollePock_CVX_theta_vs_sigtau_bounds.tex <==
x-axis,a,b
0.5,0.03,7.5
0.51,0.04,7.19
0.52,0.04,6.89
0.53,0.04,6.61
0.54,0.04,6.35
0.55,0.04,6.11
0.56,0.04,5.87
0.57,0.04,5.65
0.58,0.04,5.44
0.59,0.05,5.24
0.6,0.05,5.05
0.61,0.05,4.87
0.62,0.05,4.7
0.63,0.05,4.53
0.64,0.05,4.38
0.65,0.05,4.23
0.66,0.06,4.09
0.67,0.06,3.95
0.68,0.06,3.82
0.69,0.06,3.7
0.7,0.06,3.58
0.71,0.06,3.46
0.72,0.06,3.35
0.73,0.07,3.25
0.74,0.07,3.15
0.75,0.07,3.05
0.76,0.07,2.96
0.77,0.07,2.87
0.78,0.07,2.78
0.79,0.08,2.7
0.8,0.08,2.62
0.81,0.08,2.54
0.82,0.08,2.47
0.83,0.08,2.4
0.84,0.08,2.33
0.85,0.09,2.26
0.86,0.09,2.2
0.87,0.09,2.14
0.88,0.09,2.08
0.89,0.09,2.02
0.9,0.1,1.96
0.91,0.1,1.91
0.92,0.1,1.86
0.93,0.1,1.81
0.94,0.1,1.76
0.95,0.11,1.71
0.96,0.11,1.67
0.97,0.11,1.62
0.98,0.11,1.58
0.99,0.11,1.54
1,0.12,1.5
1.01,0.12,1.46
1.02,0.12,1.42
1.03,0.12,1.38
1.04,0.12,1.34
1.05,0.13,1.31
1.06,0.13,1.27
1.07,0.13,1.24
1.08,0.13,1.21
1.09,0.14,1.18
1.1,0.14,1.15
1.11,0.14,1.12
1.12,0.14,1.09
1.13,0.15,1.06
1.14,0.15,1.03
1.15,0.15,1.01
1.16,0.15,0.98
1.17,0.16,0.96
1.18,0.16,0.93
1.19,0.16,0.91
1.2,0.16,0.88
1.21,0.17,0.86
1.22,0.17,0.84
1.23,0.17,0.82
1.24,0.18,0.8
1.25,0.18,0.78
1.26,0.18,0.75
1.27,0.19,0.74
1.28,0.19,0.72
1.29,0.19,0.7
1.3,0.2,0.68
1.31,0.2,0.66
1.32,0.2,0.64
1.33,0.21,0.63
1.34,0.21,0.61
1.35,0.21,0.59
1.36,0.22,0.58
1.37,0.22,0.56
1.38,0.23,0.55
1.39,0.23,0.53
1.4,0.24,0.52
1.41,0.24,0.5
1.42,0.25,0.49
1.43,0.25,0.47
1.44,0.26,0.46
1.45,0.27,0.45
1.46,0.27,0.429999999999999
1.47,0.28,0.419999999999999
1.48,0.29,0.409999999999999
1.49,0.3,0.389999999999999
1.5,0.32,0.369999999999999
1.501,0.32,0.37
1.502,0.33,0.36
1.503,0.33,0.36
1.504,0.33,0.36
1.505,0.34,0.35


==> ChambollePock_CVX_theta_vs_sigtau_bounds_restrictedLyapunov.tex <==
x-axis,a
0.5,1
0.51,1
0.52,1
0.53,1
0.54,1
0.55,1
0.56,1
0.57,1
0.58,1
0.59,1
0.6,1
0.61,1
0.62,1
0.63,1
0.64,1
0.65,1
0.66,1
0.67,1
0.68,1
0.69,1
0.7,1
0.71,1
0.72,1
0.73,1
0.74,1
0.75,1
0.76,1
0.77,1
0.78,1
0.79,1
0.8,1
0.81,1
0.82,1
0.83,1
0.84,1
0.85,1
0.86,1
0.87,1
0.88,1
0.89,1
0.9,1
0.91,1
0.92,1
0.93,1
0.94,1
0.95,1
0.96,1
0.97,1
0.98,1
0.99,1


==> ChambollePock_linear_full_region.tex <==
sigtau,theta,rho
0.5,-0.14,1
0.5,0.638,0.9609375
0.5,1.416,0.9625
0.5,2.194,0.9625
0.5,2.972,0.9625
0.5,3.75,0.9625
0.5,4.528,0.9625
0.5,5.306,0.9640625
0.5,6.084,0.9640625
0.5,6.862,0.9640625
0.5,7.64,1
0.55,-0.12,0.9984375
0.55,0.515,0.9578125
0.55,1.15,0.9578125
0.55,1.785,0.9578125
0.55,2.42,0.959375
0.55,3.055,0.959375
0.55,3.69,0.959375
0.55,4.325,0.959375
0.55,4.96,0.959375
0.55,5.595,0.9609375
0.55,6.23,0.99375
0.6,-0.11,0.9984375
0.6,0.418,0.9546875
0.6,0.946,0.9546875
0.6,1.474,0.9546875
0.6,2.002,0.9546875
0.6,2.53,0.9546875
0.6,3.058,0.95625
0.6,3.586,0.95625
0.6,4.114,0.95625
0.6,4.642,0.95625
0.6,5.17,0.9984375
0.65,-0.1,0.996875
0.65,0.344,0.95
0.65,0.788,0.9484375
0.65,1.232,0.95
0.65,1.676,0.95
0.65,2.12,0.9515625
0.65,2.564,0.9515625
0.65,3.008,0.9515625
0.65,3.452,0.9515625
0.65,3.896,0.953125
0.65,4.34,0.9984375
0.7,-0.1,1
0.7,0.278,0.946875
0.7,0.656,0.946875
0.7,1.034,0.946875
0.7,1.412,0.946875
0.7,1.79,0.946875
0.7,2.168,0.9484375
0.7,2.546,0.9484375
0.7,2.924,0.9484375
0.7,3.302,0.9484375
0.7,3.68,0.9984375
0.75,-0.09,0.9984375
0.75,0.233,0.9421875
0.75,0.556,0.9421875
0.75,0.879,0.94375
0.75,1.202,0.94375
0.75,1.525,0.94375
0.75,1.848,0.94375
0.75,2.171,0.94375
0.75,2.494,0.9453125
0.75,2.817,0.9453125
0.75,3.14,0.9890625
0.8,-0.08,0.9953125
0.8,0.199,0.9390625
0.8,0.478,0.9390625
0.8,0.757,0.9390625
0.8,1.036,0.9390625
0.8,1.315,0.940625
0.8,1.594,0.940625
0.8,1.873,0.940625
0.8,2.152,0.940625
0.8,2.431,0.940625
0.8,2.71,0.996875
0.85,-0.08,0.9984375
0.85,0.163,0.9359375
0.85,0.406,0.9359375
0.85,0.649,0.9359375
0.85,0.891999999999999,0.9359375
0.85,1.135,0.9359375
0.85,1.378,0.9359375
0.85,1.621,0.9375
0.85,1.864,0.9375
0.85,2.107,0.9375
0.85,2.35,0.9984375
0.9,-0.07,0.99375
0.9,0.141,0.93125
0.9,0.352,0.93125
0.9,0.563,0.93125
0.9,0.773999999999999,0.9328125
0.9,0.984999999999999,0.9328125
0.9,1.196,0.9328125
0.9,1.407,0.9328125
0.9,1.618,0.9328125
0.9,1.829,0.9328125
0.9,2.04,0.9875
0.95,-0.07,0.996875
0.95,0.116,0.928125
0.95,0.302,0.928125
0.95,0.488,0.928125
0.95,0.673999999999999,0.928125
0.95,0.859999999999999,0.928125
0.95,1.046,0.928125
0.95,1.232,0.9296875
0.95,1.418,0.9296875
0.95,1.604,0.9296875
0.95,1.79,1
1,-0.06,0.9921875
1,0.103,0.9234375
1,0.266,0.925
1,0.429,0.925
1,0.591999999999999,0.925
1,0.754999999999999,0.925
1,0.917999999999999,0.925
1,1.081,0.925
1,1.244,0.925
1,1.407,0.9265625
1,1.57,1
1.05,-0.06,0.996875
1.05,0.0839999999999998,0.9203125
1.05,0.228,0.9203125
1.05,0.371999999999999,0.9203125
1.05,0.515999999999999,0.9203125
1.05,0.659999999999999,0.921875
1.05,0.803999999999999,0.921875
1.05,0.947999999999999,0.921875
1.05,1.092,0.921875
1.05,1.236,0.921875
1.05,1.38,0.996875
1.1,-0.05,0.99375
1.1,0.0759999999999998,0.9171875
1.1,0.202,0.9171875
1.1,0.327999999999999,0.9171875
1.1,0.453999999999999,0.9171875
1.1,0.579999999999999,0.915625
1.1,0.705999999999999,0.9171875
1.1,0.831999999999999,0.9171875
1.1,0.957999999999998,0.91875
1.1,1.084,0.91875
1.1,1.21,0.9796875
1.15,-0.05,1
1.15,0.0619999999999998,0.9140625
1.15,0.174,0.9125
1.15,0.285999999999999,0.9140625
1.15,0.397999999999999,0.9140625
1.15,0.509999999999999,0.9140625
1.15,0.621999999999999,0.9140625
1.15,0.733999999999999,0.9140625
1.15,0.845999999999998,0.9140625
1.15,0.957999999999998,0.9140625
1.15,1.07,0.9859375
1.2,-0.04,0.9984375
1.2,0.058,0.9171875
1.2,0.156,0.909375
1.2,0.254,0.909375
1.2,0.352,0.909375
1.2,0.45,0.9109375
1.2,0.548,0.9109375
1.2,0.646,0.9109375
1.2,0.744,0.9109375
1.2,0.842,0.909375
1.2,0.94,0.9703125
1.25,-0.03,0.996875
1.25,0.056,0.9203125
1.25,0.142,0.90625
1.25,0.228,0.90625
1.25,0.314,0.90625
1.25,0.4,0.90625
1.25,0.486,0.90625
1.25,0.572,0.90625
1.25,0.658,0.9078125
1.25,0.744,0.9078125
1.25,0.83,0.971875
1.3,-0.02,0.996875
1.3,0.055,0.925
1.3,0.13,0.9015625
1.3,0.205,0.903125
1.3,0.28,0.9015625
1.3,0.355,0.903125
1.3,0.43,0.903125
1.3,0.505,0.903125
1.3,0.58,0.903125
1.3,0.655,0.903125
1.3,0.73,0.9609375
1.35,-0.01,0.996875
1.35,0.056,0.93125
1.35,0.122,0.8984375
1.35,0.188,0.8984375
1.35,0.254,0.8984375
1.35,0.32,0.9
1.35,0.386,0.9
1.35,0.452,0.9
1.35,0.518,0.9
1.35,0.584,0.9
1.35,0.65,1
1.4,3.46944695195361e-18,0.9984375
1.4,0.057,0.9390625
1.4,0.114,0.896875
1.4,0.171,0.8953125
1.4,0.228,0.8953125
1.4,0.285,0.8953125
1.4,0.342,0.8953125
1.4,0.399,0.8953125
1.4,0.456,0.8953125
1.4,0.513,0.896875
1.4,0.57,0.9953125
1.45,0.02,0.990625
1.45,0.068,0.940625
1.45,0.116,0.9
1.45,0.164,0.8921875
1.45,0.212,0.8921875
1.45,0.26,0.890625
1.45,0.308,0.890625
1.45,0.356,0.890625
1.45,0.404,0.8921875
1.45,0.452,0.8921875
1.45,0.5,0.9984375
1.5,0.03,0.9953125
1.5,0.07,0.9515625
1.5,0.11,0.9140625
1.5,0.15,0.8890625
1.5,0.19,0.8859375
1.5,0.23,0.8890625
1.5,0.27,0.8890625
1.5,0.31,0.8890625
1.5,0.35,0.8890625
1.5,0.39,0.8890625
1.5,0.429999999999999,0.9484375
1.55,0.05,0.9921875
1.55,0.082,0.9578125
1.55,0.114,0.925
1.55,0.146,0.9
1.55,0.178,0.884375
1.55,0.21,0.884375
1.55,0.242,0.884375
1.55,0.274,0.884375
1.55,0.306,0.8859375
1.55,0.338,0.8859375
1.55,0.369999999999999,0.9234375
1.6,0.07,0.99375
1.6,0.0949999999999999,0.9671875
1.6,0.12,0.9421875
1.6,0.145,0.9203125
1.6,0.17,0.9015625
1.6,0.195,0.8875
1.6,0.22,0.88125
1.6,0.245,0.88125
1.6,0.27,0.88125
1.6,0.294999999999999,0.88125
1.6,0.319999999999999,0.9421875
1.65,0.1,0.990625
1.65,0.117,0.9765625
1.65,0.134,0.9609375
1.65,0.151,0.9484375
1.65,0.168,0.9359375
1.65,0.185,0.9265625
1.65,0.202,0.9203125
1.65,0.219,0.9171875
1.65,0.235999999999999,0.9203125
1.65,0.252999999999999,0.9328125
1.65,0.269999999999999,0.975
1.7,0.15,1
1.7,0.155,0.996875
1.7,0.16,0.9953125
1.7,0.165,0.99375
1.7,0.17,0.99375
1.7,0.175,0.9921875
1.7,0.18,0.9921875
1.7,0.185,0.99375
1.7,0.189999999999999,0.9953125
1.7,0.194999999999999,0.996875
1.7,0.199999999999999,1


==> DR_linear_sigmaEq1_betaEq2_lambdaEq1.tex <==
x-axis,a,b
0.010000,0.980488,0.980296
0.060404,0.889759,0.889318
0.110808,0.810736,0.810442
0.161212,0.742445,0.741612
0.211616,0.681959,0.681193
0.262020,0.628302,0.627867
0.312424,0.581474,0.580566
0.362828,0.538548,0.538416
0.413232,0.501476,0.500695
0.463636,0.467330,0.466803
0.514040,0.437087,0.436240
0.564444,0.408795,0.408582
0.614848,0.384405,0.383474
0.665253,0.360991,0.360612
0.715657,0.347333,0.346567
0.766061,0.366845,0.366115
0.816465,0.385381,0.384642
0.866869,0.402941,0.402210
0.917273,0.419526,0.418880
0.967677,0.435136,0.434710
1.018081,0.449770,0.449754
1.068485,0.464403,0.464062
1.118889,0.478062,0.477683
1.169293,0.490744,0.490661
1.219697,0.503427,0.503037
1.270101,0.515134,0.514850
1.320505,0.526841,0.526134
1.370909,0.537572,0.536923
1.421313,0.547328,0.547247
1.471717,0.558060,0.557134
1.522121,0.566840,0.566610
1.572525,0.576596,0.575699
1.622929,0.585376,0.584424
1.673333,0.593181,0.592806
1.723737,0.600985,0.600863
1.774141,0.608790,0.608613
1.824545,0.616595,0.616075
1.874949,0.623424,0.623262
1.925354,0.630253,0.630189
1.975758,0.637082,0.636870
2.026162,0.643911,0.643318
2.076566,0.649765,0.649544
2.126970,0.655618,0.655560
2.177374,0.661472,0.661375
2.227778,0.667325,0.667000
2.278182,0.673179,0.672443
2.328586,0.678057,0.677713
2.378990,0.682935,0.682818
2.429394,0.687812,0.687765
2.479798,0.692690,0.692562
2.530202,0.697568,0.697216
2.580606,0.702446,0.701732
2.631010,0.706349,0.706116
2.681414,0.711227,0.710375
2.731818,0.715129,0.714512
2.782222,0.719031,0.718535
2.832626,0.722934,0.722446
2.883030,0.726836,0.726251
2.933434,0.730738,0.729954
2.983838,0.733665,0.733558
3.034242,0.737567,0.737069
3.084646,0.740494,0.740488
3.135051,0.744396,0.743821
3.185455,0.747323,0.747069
3.235859,0.750250,0.750237
3.286263,0.754152,0.753326
3.336667,0.757079,0.756341
3.387071,0.760006,0.759283
3.437475,0.762933,0.762155
3.487879,0.765859,0.764960
3.538283,0.767811,0.767700
3.588687,0.770737,0.770377
3.639091,0.773664,0.772994
3.689495,0.775615,0.775551
3.739899,0.778542,0.778052
3.790303,0.781469,0.780498
3.840707,0.783420,0.782891
3.891111,0.785371,0.785233
3.941515,0.788298,0.787525
3.991919,0.790249,0.789768
4.042323,0.792200,0.791965
4.092727,0.794151,0.794117
4.143131,0.797078,0.796224
4.193535,0.799029,0.798290
4.243939,0.800980,0.800313
4.294343,0.802932,0.802297
4.344747,0.804883,0.804242
4.395152,0.806834,0.806149
4.445556,0.808785,0.808020
4.495960,0.810736,0.809854
4.546364,0.811712,0.811655
4.596768,0.813663,0.813421
4.647172,0.815614,0.815155
4.697576,0.817565,0.816857
4.747980,0.818541,0.818528
4.798384,0.820492,0.820169
4.848788,0.822443,0.821780
4.899192,0.823419,0.823363
4.949596,0.825370,0.824918
5.000000,0.827321,0.826446


==> DY_linear_rate6.tex <==
x-axis,a,b,c
1.000000,0.250750,0.777778,0.500000
1.393939,0.250750,0.826371,0.500000
1.787879,0.259530,0.860608,0.500000
2.181818,0.294651,0.885633,0.521739
2.575758,0.333675,0.904478,0.562914
2.969697,0.369771,0.919021,0.597561
3.363636,0.402941,0.930480,0.627119
3.757576,0.434160,0.939668,0.652632
4.151515,0.462452,0.947147,0.674877
4.545455,0.488793,0.953318,0.694444
4.939394,0.512207,0.958468,0.711790
5.333333,0.533670,0.962810,0.727273
5.727273,0.553182,0.966505,0.741176
6.121212,0.571718,0.969676,0.753731
6.515152,0.589278,0.972417,0.765125
6.909091,0.604888,0.974802,0.775510
7.303030,0.619521,0.976891,0.785016
7.696970,0.633180,0.978730,0.793750
8.090909,0.648789,0.980359,0.801802
8.484848,0.657569,0.981807,0.809249
8.878788,0.668301,0.983101,0.816156
9.272727,0.679032,0.984261,0.822581
9.666667,0.688788,0.985306,0.828571
10.060606,0.697568,0.986250,0.834171
10.454545,0.706349,0.987106,0.839416
10.848485,0.714153,0.987885,0.844340
11.242424,0.721958,0.988595,0.848970
11.636364,0.729763,0.989244,0.853333
12.030303,0.736592,0.989840,0.857451
12.424242,0.743421,0.990387,0.861345
12.818182,0.749274,0.990892,0.865031
13.212121,0.756104,0.991357,0.868526
13.606061,0.760981,0.991788,0.871845
14.000000,0.766835,0.992188,0.875000
14.393939,0.771713,0.992558,0.878004
14.787879,0.777566,0.992904,0.880866
15.181818,0.781469,0.993225,0.883598
15.575758,0.786347,0.993526,0.886207
15.969697,0.791225,0.993806,0.888702
16.363636,0.795127,0.994069,0.891089
16.757576,0.799029,0.994316,0.893376
17.151515,0.802932,0.994547,0.895570
17.545455,0.806834,0.994765,0.897674
17.939394,0.810736,0.994970,0.899696
18.333333,0.813663,0.995163,0.901639
18.727273,0.817565,0.995345,0.903509
19.121212,0.820492,0.995517,0.905308
19.515152,0.823419,0.995679,0.907042
19.909091,0.826346,0.995833,0.908714
20.303030,0.829272,0.995979,0.910326
20.696970,0.832199,0.996118,0.911883
21.090909,0.835126,0.996249,0.913386
21.484848,0.838053,0.996374,0.914839
21.878788,0.840004,0.996492,0.916244
22.272727,0.842931,0.996605,0.917603
22.666667,0.844882,0.996713,0.918919
23.060606,0.847809,0.996815,0.920193
23.454545,0.849760,0.996913,0.921429
23.848485,0.851711,0.997007,0.922626
24.242424,0.853662,0.997096,0.923788
24.636364,0.856589,0.997181,0.924915
25.030303,0.858540,0.997263,0.926009
25.424242,0.860491,0.997341,0.927072
25.818182,0.862442,0.997416,0.928105
26.212121,0.864394,0.997487,0.929108
26.606061,0.865369,0.997556,0.930085
27.000000,0.867320,0.997622,0.931034
27.393939,0.869271,0.997685,0.931959
27.787879,0.871223,0.997746,0.932859
28.181818,0.872198,0.997804,0.933735
28.575758,0.874149,0.997861,0.934589
28.969697,0.876101,0.997915,0.935421
29.363636,0.877076,0.997967,0.936232
29.757576,0.879027,0.998017,0.937023
30.151515,0.880003,0.998065,0.937795
30.545455,0.881954,0.998112,0.938547
30.939394,0.882930,0.998157,0.939282
31.333333,0.883905,0.998200,0.940000
31.727273,0.885856,0.998242,0.940701
32.121212,0.886832,0.998282,0.941385
32.515152,0.887808,0.998321,0.942054
32.909091,0.889759,0.998359,0.942708
33.303030,0.890734,0.998395,0.943348
33.696970,0.891710,0.998430,0.943973
34.090909,0.892686,0.998465,0.944584
34.484848,0.893661,0.998498,0.945183
34.878788,0.894637,0.998529,0.945768
35.272727,0.896588,0.998560,0.946341
35.666667,0.897563,0.998590,0.946903
36.060606,0.898539,0.998619,0.947452
36.454545,0.899515,0.998648,0.947991
36.848485,0.900490,0.998675,0.948518
37.242424,0.901466,0.998701,0.949035
37.636364,0.902441,0.998727,0.949541
38.030303,0.903417,0.998752,0.950038
38.424242,0.904393,0.998776,0.950525
38.818182,0.905368,0.998800,0.951002
39.212121,0.906344,0.998822,0.951471
39.606061,0.906344,0.998845,0.951930
40.000000,0.907319,0.998866,0.952381


==> Heavy-ball_linear_Ghadimi.tex <==
x-axis,a
0.005025,0.818926
0.015075,0.820397
0.025126,0.821844
0.035176,0.823268
0.045226,0.824670
0.055276,0.826049
0.065327,0.827407
0.075377,0.828744
0.085427,0.830060
0.095477,0.831356
0.105528,0.832632
0.115578,0.833890
0.125628,0.835128
0.135678,0.836349
0.145729,0.837551
0.155779,0.838736
0.165829,0.839903
0.175879,0.841054
0.185930,0.842189
0.195980,0.843307
0.206030,0.844410
0.216080,0.845497
0.226131,0.847458
0.236181,0.858661
0.246231,0.869215
0.256281,0.879173
0.266332,0.888584
0.276382,0.897493
0.286432,0.905938
0.296482,0.913956
0.306533,0.921577
0.316583,0.928830
0.326633,0.935741
0.336683,0.942335
0.346734,0.948631
0.356784,0.954651
0.366834,0.960411
0.376884,0.965929
0.386935,0.971219
0.396985,0.976295
0.407035,0.981169
0.417085,0.985855
0.427136,0.990361
0.437186,0.994699
0.447236,0.998878


==> Heavy-ball_linear_PEP.tex <==
x-axis,a
-0.497487,0.994146
-0.487437,0.966830
-0.477387,0.940489
-0.467337,0.921953
-0.457286,0.888783
-0.447236,0.870247
-0.437186,0.869271
-0.427136,0.868296
-0.417085,0.867320
-0.407035,0.866345
-0.396985,0.865369
-0.386935,0.864394
-0.376884,0.863418
-0.366834,0.862442
-0.356784,0.861467
-0.346734,0.860491
-0.336683,0.859516
-0.326633,0.858540
-0.316583,0.856589
-0.306533,0.855613
-0.296482,0.854638
-0.286432,0.853662
-0.276382,0.852687
-0.266332,0.851711
-0.256281,0.849760
-0.246231,0.848784
-0.236181,0.847809
-0.226131,0.846833
-0.216080,0.844882
-0.206030,0.843906
-0.195980,0.842931
-0.185930,0.840979
-0.175879,0.840004
-0.165829,0.838053
-0.155779,0.837077
-0.145729,0.835126
-0.135678,0.834150
-0.125628,0.832199
-0.115578,0.831224
-0.105528,0.829272
-0.095477,0.827321
-0.085427,0.826346
-0.075377,0.824395
-0.065327,0.822443
-0.055276,0.820492
-0.045226,0.819517
-0.035176,0.817565
-0.025126,0.815614
-0.015075,0.813663
-0.005025,0.811712
0.005025,0.809761
0.015075,0.807810
0.025126,0.804883
0.035176,0.802932
0.045226,0.800980
0.055276,0.799029
0.065327,0.796103
0.075377,0.794151
0.085427,0.791225
0.095477,0.789273
0.105528,0.786347
0.115578,0.783420
0.125628,0.780493
0.135678,0.778542
0.145729,0.775615
0.155779,0.771713
0.165829,0.768786
0.175879,0.765859
0.185930,0.762933
0.195980,0.759030
0.206030,0.755128
0.216080,0.752201
0.226131,0.748299
0.236181,0.744396
0.246231,0.739519
0.256281,0.735616
0.266332,0.730738
0.276382,0.726836
0.286432,0.720982
0.296482,0.716104
0.306533,0.711227
0.316583,0.705373
0.326633,0.699520
0.336683,0.692690
0.346734,0.685861
0.356784,0.679032
0.366834,0.671228
0.376884,0.662447
0.386935,0.653667
0.396985,0.643911
0.407035,0.633180
0.417085,0.620497
0.427136,0.606839
0.437186,0.612692
0.447236,0.621473
0.457286,0.630253
0.467337,0.639033
0.477387,0.647813
0.487437,0.656594
0.497487,0.665374
0.507538,0.674154
0.517588,0.683910
0.527638,0.692690
0.537688,0.701471
0.547739,0.710251
0.557789,0.719031
0.567839,0.728787
0.577889,0.737567
0.587940,0.746348
0.597990,0.755128
0.608040,0.764884
0.618090,0.773664
0.628141,0.782444
0.638191,0.791225
0.648241,0.800980
0.658291,0.809761
0.668342,0.818541
0.678392,0.827321
0.688442,0.837077
0.698492,0.845857
0.708543,0.854638
0.718593,0.863418
0.728643,0.872198
0.738693,0.881954
0.748744,0.890734
0.758794,0.899515
0.768844,0.908295
0.778894,0.917075
0.788945,0.925855
0.798995,0.934636
0.809045,0.944392
0.819095,0.953172
0.829146,0.961952
0.839196,0.970732
0.849246,0.979513
0.859296,0.988293
0.869347,0.997073


==> Polyakgrad_CVX_params.tex <==
x-axis,a
-1,0
-0.99,0.02109375
-0.98,0.0421875
-0.97,0.06064453125
-0.96,0.08173828125
-0.95,0.1001953125
-0.94,0.1212890625
-0.93,0.1423828125
-0.92,0.16083984375
-0.91,0.18193359375
-0.9,0.200390625
-0.89,0.221484375
-0.88,0.242578125
-0.87,0.26103515625
-0.86,0.28212890625
-0.85,0.3005859375
-0.84,0.3216796875
-0.83,0.34013671875
-0.82,0.36123046875
-0.81,0.38232421875
-0.8,0.40078125
-0.79,0.421875
-0.78,0.44033203125
-0.77,0.46142578125
-0.76,0.48251953125
-0.75,0.5009765625
-0.74,0.5220703125
-0.73,0.54052734375
-0.72,0.56162109375
-0.71,0.580078125
-0.7,0.601171875
-0.69,0.622265625
-0.68,0.64072265625
-0.67,0.66181640625
-0.66,0.6802734375
-0.65,0.7013671875
-0.64,0.7224609375
-0.63,0.74091796875
-0.62,0.76201171875
-0.61,0.78046875
-0.6,0.8015625
-0.59,0.82001953125
-0.58,0.84111328125
-0.57,0.86220703125
-0.56,0.8806640625
-0.55,0.9017578125
-0.54,0.92021484375
-0.53,0.94130859375
-0.52,0.96240234375
-0.51,0.980859375
-0.5,1.001953125
-0.49,1.02041015625
-0.48,1.04150390625
-0.47,1.06259765625
-0.46,1.0810546875
-0.45,1.1021484375
-0.44,1.12060546875
-0.43,1.14169921875
-0.42,1.16015625
-0.41,1.18125
-0.4,1.20234375
-0.39,1.22080078125
-0.38,1.24189453125
-0.37,1.2603515625
-0.36,1.2814453125
-0.35,1.3025390625
-0.34,1.32099609375
-0.33,1.34208984375
-0.32,1.360546875
-0.31,1.381640625
-0.3,1.40009765625
-0.29,1.42119140625
-0.28,1.44228515625
-0.27,1.4607421875
-0.26,1.4818359375
-0.25,1.50029296875
-0.24,1.52138671875
-0.23,1.54248046875
-0.22,1.5609375
-0.21,1.58203125
-0.2,1.60048828125
-0.19,1.62158203125
-0.18,1.6400390625
-0.17,1.6611328125
-0.16,1.6822265625
-0.15,1.70068359375
-0.14,1.72177734375
-0.13,1.740234375
-0.12,1.761328125
-0.11,1.782421875
-0.1,1.80087890625
-0.09,1.82197265625
-0.08,1.8404296875
-0.07,1.8615234375
-0.0599999999999999,1.8826171875
-0.0499999999999999,1.90107421875
-0.04,1.92216796875
-0.03,1.940625
-0.02,1.96171875
-0.01,1.98017578125
0,2.00126953125
0.01,2.02236328125
0.02,2.0408203125
0.03,2.0619140625
0.04,2.08037109375
0.0499999999999999,2.10146484375
0.0599999999999999,2.12255859375
0.07,2.141015625
0.08,2.162109375
0.09,2.18056640625
0.1,2.20166015625
0.11,2.2201171875
0.12,2.2412109375
0.13,2.2623046875
0.14,2.28076171875
0.15,2.30185546875
0.16,2.3203125
0.17,2.34140625
0.18,2.3625
0.19,2.38095703125
0.2,2.40205078125
0.21,2.4205078125
0.22,2.4416015625
0.23,2.46005859375
0.24,2.48115234375
0.25,2.499609375
0.26,2.5154296875
0.27,2.53125
0.28,2.54443359375
0.29,2.5576171875
0.3,2.5681640625
0.31,2.57607421875
0.32,2.583984375
0.33,2.5892578125
0.34,2.59453125
0.35,2.59716796875
0.36,2.5998046875
0.37,2.5998046875
0.38,2.59716796875
0.39,2.59453125
0.4,2.59189453125
0.41,2.58662109375
0.42,2.5787109375
0.43,2.57080078125
0.44,2.56025390625
0.45,2.54970703125
0.46,2.53916015625
0.47,2.52333984375
0.48,2.51015625
0.49,2.4943359375
0.5,2.47587890625
0.51,2.457421875
0.52,2.436328125
0.53,2.415234375
0.54,2.394140625
0.55,2.3677734375
0.56,2.34404296875
0.57,2.31767578125
0.58,2.288671875
0.59,2.25966796875
0.6,2.2306640625
0.61,2.1990234375
0.62,2.16474609375
0.63,2.13046875
0.64,2.09619140625
0.65,2.05927734375
0.66,2.02236328125
0.67,1.9828125
0.68,1.940625
0.69,1.90107421875
0.7,1.85625
0.71,1.8140625
0.72,1.7666015625
0.73,1.72177734375
0.74,1.6716796875
0.75,1.62421875
0.76,1.57412109375
0.77,1.52138671875
0.78,1.46865234375
0.79,1.41591796875
0.8,1.360546875
0.81,1.3025390625
0.82,1.24716796875
0.83,1.1865234375
0.84,1.12587890625
0.85,1.065234375
0.86,1.00458984375
0.87,0.938671875
0.88,0.875390625
0.89,0.80947265625
0.9,0.74091796875
0.91,0.67236328125
0.92,0.60380859375
0.93,0.5326171875
0.94,0.4587890625
0.95,0.38759765625
0.96,0.3211328125
0.97,0.23466796875
0.98,0.158203125
0.99,0.08173828125
1,0


==> Polyakgrad_Ghadimi.tex <==
x-axis,a
0,2
0.01,1.98
0.02,1.96
0.03,1.94
0.04,1.92
0.05,1.9
0.06,1.88
0.07,1.86
0.08,1.84
0.09,1.82
0.1,1.8
0.11,1.78
0.12,1.76
0.13,1.74
0.14,1.72
0.15,1.7
0.16,1.68
0.17,1.66
0.18,1.64
0.19,1.62
0.2,1.6
0.21,1.58
0.22,1.56
0.23,1.54
0.24,1.52
0.25,1.5
0.26,1.48
0.27,1.46
0.28,1.44
0.29,1.42
0.3,1.4
0.31,1.38
0.32,1.36
0.33,1.34
0.34,1.32
0.35,1.3
0.36,1.28
0.37,1.26
0.38,1.24
0.39,1.22
0.4,1.2
0.41,1.18
0.42,1.16
0.43,1.14
0.44,1.12
0.45,1.1
0.46,1.08
0.47,1.06
0.48,1.04
0.49,1.02
0.5,1
0.51,0.98
0.52,0.96
0.53,0.94
0.54,0.92
0.55,0.9
0.56,0.88
0.57,0.86
0.58,0.84
0.59,0.82
0.6,0.8
0.61,0.78
0.62,0.76
0.63,0.74
0.64,0.72
0.65,0.7
0.66,0.68
0.67,0.66
0.68,0.64
0.69,0.62
0.7,0.6
0.71,0.58
0.72,0.56
0.73,0.54
0.74,0.52
0.75,0.5
0.76,0.48
0.77,0.46
0.78,0.44
0.79,0.42
0.8,0.4
0.81,0.38
0.82,0.36
0.83,0.34
0.84,0.32
0.85,0.3
0.86,0.28
0.87,0.26
0.88,0.24
0.89,0.22
0.9,0.2
0.91,0.18
0.92,0.16
0.93,0.14
0.94,0.12
0.95,0.1
0.96,0.0800000000000001
0.97,0.0600000000000001
0.98,0.04
0.99,0.02
1,0


==> Polyakgrad_cvx_params_JohanssonGhadimi_our_rho1.tex <==
x-axis,a,b
0,2,2.00126953125
0.01,1.98,2.02236328125
0.02,1.96,2.0408203125
0.03,1.94,2.0619140625
0.04,1.92,2.08037109375
0.05,1.9,2.10146484375
0.06,1.88,2.12255859375
0.07,1.86,2.141015625
0.08,1.84,2.162109375
0.09,1.82,2.18056640625
0.1,1.8,2.20166015625
0.11,1.78,2.2201171875
0.12,1.76,2.2412109375
0.13,1.74,2.2623046875
0.14,1.72,2.28076171875
0.15,1.7,2.30185546875
0.16,1.68,2.3203125
0.17,1.66,2.34140625
0.18,1.64,2.3625
0.19,1.62,2.38095703125
0.2,1.6,2.40205078125
0.21,1.58,2.4205078125
0.22,1.56,2.4416015625
0.23,1.54,2.46005859375
0.24,1.52,2.48115234375
0.25,1.5,2.499609375
0.26,1.48,2.5154296875
0.27,1.46,2.53125
0.28,1.44,2.54443359375
0.29,1.42,2.5576171875
0.3,1.4,2.5681640625
0.31,1.38,2.57607421875
0.32,1.36,2.583984375
0.33,1.34,2.5892578125
0.34,1.32,2.59453125
0.35,1.3,2.59716796875
0.36,1.28,2.5998046875
0.37,1.26,2.5998046875
0.38,1.24,2.59716796875
0.39,1.22,2.59453125
0.4,1.2,2.59189453125
0.41,1.18,2.58662109375
0.42,1.16,2.5787109375
0.43,1.14,2.57080078125
0.44,1.12,2.56025390625
0.45,1.1,2.54970703125
0.46,1.08,2.53916015625
0.47,1.06,2.52333984375
0.48,1.04,2.51015625
0.49,1.02,2.4943359375
0.5,1,2.47587890625
0.51,0.98,2.457421875
0.52,0.96,2.436328125
0.53,0.94,2.415234375
0.54,0.92,2.394140625
0.55,0.9,2.3677734375
0.56,0.88,2.34404296875
0.57,0.86,2.31767578125
0.58,0.84,2.288671875
0.59,0.82,2.25966796875
0.6,0.8,2.2306640625
0.61,0.78,2.1990234375
0.62,0.76,2.16474609375
0.63,0.74,2.13046875
0.64,0.72,2.09619140625
0.65,0.7,2.05927734375
0.66,0.68,2.02236328125
0.67,0.66,1.9828125
0.68,0.64,1.940625
0.69,0.62,1.90107421875
0.7,0.6,1.85625
0.71,0.58,1.8140625
0.72,0.56,1.7666015625
0.73,0.54,1.72177734375
0.74,0.52,1.6716796875
0.75,0.5,1.62421875
0.76,0.48,1.57412109375
0.77,0.46,1.52138671875
0.78,0.44,1.46865234375
0.79,0.42,1.41591796875
0.8,0.4,1.360546875
0.81,0.38,1.3025390625
0.82,0.36,1.24716796875
0.83,0.34,1.1865234375
0.84,0.32,1.12587890625
0.85,0.3,1.065234375
0.86,0.28,1.00458984375
0.87,0.26,0.938671875
0.88,0.24,0.875390625
0.89,0.22,0.80947265625
0.9,0.2,0.74091796875
0.91,0.18,0.67236328125
0.92,0.16,0.60380859375
0.93,0.14,0.5326171875
0.94,0.12,0.4587890625
0.95,0.1,0.3849609375
0.96,0.0800000000000001,0.319814453125
0.97,0.0600000000000001,0.23466796875
0.98,0.04,0.158203125
0.99,0.02,0.08173828125
1,0,0


==> Polyakproxgrad_CVX_params_sweep_delta1_delta2_0.tex <==
x-axis,a
-1,0
-0.99,0.02109375
-0.98,0.0421875
-0.97,0.06064453125
-0.96,0.08173828125
-0.95,0.1001953125
-0.94,0.1212890625
-0.93,0.1423828125
-0.92,0.16083984375
-0.91,0.18193359375
-0.9,0.200390625
-0.89,0.221484375
-0.88,0.242578125
-0.87,0.26103515625
-0.86,0.28212890625
-0.85,0.3005859375
-0.84,0.3216796875
-0.83,0.34013671875
-0.82,0.36123046875
-0.81,0.38232421875
-0.8,0.40078125
-0.79,0.421875
-0.78,0.44033203125
-0.77,0.46142578125
-0.76,0.48251953125
-0.75,0.5009765625
-0.74,0.5220703125
-0.73,0.54052734375
-0.72,0.56162109375
-0.71,0.580078125
-0.7,0.601171875
-0.69,0.622265625
-0.68,0.64072265625
-0.67,0.66181640625
-0.66,0.6802734375
-0.65,0.7013671875
-0.64,0.7224609375
-0.63,0.74091796875
-0.62,0.76201171875
-0.61,0.78046875
-0.6,0.8015625
-0.59,0.82001953125
-0.58,0.84111328125
-0.57,0.86220703125
-0.56,0.8806640625
-0.55,0.9017578125
-0.54,0.92021484375
-0.53,0.94130859375
-0.52,0.96240234375
-0.51,0.980859375
-0.5,1.001953125
-0.49,1.02041015625
-0.48,1.04150390625
-0.47,1.0599609375
-0.46,1.0810546875
-0.45,1.1021484375
-0.44,1.12060546875
-0.43,1.14169921875
-0.42,1.16015625
-0.41,1.18125
-0.4,1.20234375
-0.39,1.22080078125
-0.38,1.24189453125
-0.37,1.2603515625
-0.36,1.2814453125
-0.35,1.3025390625
-0.34,1.32099609375
-0.33,1.34208984375
-0.32,1.360546875
-0.31,1.381640625
-0.3,1.40009765625
-0.29,1.42119140625
-0.28,1.44228515625
-0.27,1.4607421875
-0.26,1.4818359375
-0.25,1.50029296875
-0.24,1.52138671875
-0.23,1.54248046875
-0.22,1.5609375
-0.21,1.58203125
-0.2,1.60048828125
-0.19,1.62158203125
-0.18,1.6400390625
-0.17,1.6611328125
-0.16,1.6822265625
-0.15,1.70068359375
-0.14,1.72177734375
-0.13,1.740234375
-0.12,1.761328125
-0.11,1.782421875
-0.1,1.80087890625
-0.09,1.82197265625
-0.08,1.8404296875
-0.07,1.8615234375
-0.0599999999999999,1.8826171875
-0.0499999999999999,1.90107421875
-0.04,1.92216796875
-0.03,1.940625
-0.02,1.96171875
-0.01,1.98017578125
0,2.00126953125
0.01,2.02236328125
0.02,2.0408203125
0.03,2.0619140625
0.04,2.08037109375
0.0499999999999999,2.10146484375
0.0599999999999999,2.12255859375
0.07,2.141015625
0.08,2.162109375
0.09,2.18056640625
0.1,2.20166015625
0.11,2.2201171875
0.12,2.2412109375
0.13,2.2623046875
0.14,2.28076171875
0.15,2.30185546875
0.16,2.3203125
0.17,2.34140625
0.18,2.3625
0.19,2.38095703125
0.2,2.3994140625
0.21,2.41787109375
0.22,2.4310546875
0.23,2.44423828125
0.24,2.457421875
0.25,2.46533203125
0.26,2.4732421875
0.27,2.48115234375
0.28,2.4837890625
0.29,2.4890625
0.3,2.4890625
0.31,2.49169921875
0.32,2.4890625
0.33,2.4890625
0.34,2.4837890625
0.35,2.478515625
0.36,2.4732421875
0.37,2.46796875
0.38,2.457421875
0.39,2.44951171875
0.4,2.43896484375
0.41,2.42578125
0.42,2.415234375
0.43,2.3994140625
0.44,2.38623046875
0.45,2.37041015625
0.46,2.351953125
0.47,2.3361328125
0.48,2.3150390625
0.49,2.29658203125
0.5,2.27548828125
0.51,2.25439453125
0.52,2.2306640625
0.53,2.20693359375
0.54,2.183203125
0.55,2.1568359375
0.56,2.13046875
0.57,2.1041015625
0.58,2.07509765625
0.59,2.04609375
0.6,2.01708984375
0.61,1.98544921875
0.62,1.95380859375
0.63,1.92216796875
0.64,1.887890625
0.65,1.85361328125
0.66,1.8193359375
0.67,1.782421875
0.68,1.7455078125
0.69,1.70859375
0.7,1.66904296875
0.71,1.6294921875
0.72,1.58994140625
0.73,1.54775390625
0.74,1.50556640625
0.75,1.4607421875
0.76,1.4185546875
0.77,1.37373046875
0.78,1.32626953125
0.79,1.27880859375
0.8,1.23134765625
0.81,1.18125
0.82,1.13115234375
0.83,1.0810546875
0.84,1.0283203125
0.85,0.9755859375
0.86,0.92021484375
0.87,0.86484375
0.88,0.8068359375
0.89,0.748828125
0.9,0.6908203125
0.91,0.63017578125
0.92,0.56689453125
0.93,0.50361328125
0.94,0.4376953125
0.95,0.369140625
0.96,0.3005859375
0.97,0.233076171875
0.98,0.15556640625
0.99,0.0791015625
1,0


==> Polyakproxgrad_CVX_params_sweep_delta2_delta1_0.tex <==
x-axis,a
-0.53,0.00263671875
-0.52,0.0052734375
-0.51,0.00263671875
-0.5,0.010546875
-0.49,0.5220703125
-0.48,0.6908203125
-0.47,0.80419921875
-0.46,0.89384765625
-0.45,0.9650390625
-0.44,1.02568359375
-0.43,1.07578125
-0.42,1.11796875
-0.41,1.1548828125
-0.4,1.18388671875
-0.39,1.21552734375
-0.38,1.23662109375
-0.37,1.2603515625
-0.36,1.2814453125
-0.35,1.29990234375
-0.34,1.32099609375
-0.33,1.34208984375
-0.32,1.360546875
-0.31,1.381640625
-0.3,1.40009765625
-0.29,1.42119140625
-0.28,1.44228515625
-0.27,1.4607421875
-0.26,1.4818359375
-0.25,1.50029296875
-0.24,1.52138671875
-0.23,1.54248046875
-0.22,1.5609375
-0.21,1.58203125
-0.2,1.60048828125
-0.19,1.62158203125
-0.18,1.6400390625
-0.17,1.6611328125
-0.16,1.6822265625
-0.15,1.70068359375
-0.14,1.72177734375
-0.13,1.740234375
-0.12,1.761328125
-0.11,1.782421875
-0.1,1.80087890625
-0.09,1.82197265625
-0.08,1.8404296875
-0.07,1.8615234375
-0.0599999999999999,1.87998046875
-0.0499999999999999,1.90107421875
-0.04,1.92216796875
-0.03,1.940625
-0.02,1.96171875
-0.01,1.98017578125
0,2.00126953125
0.01,2.02236328125
0.02,2.0408203125
0.03,2.0619140625
0.04,2.08037109375
0.0499999999999999,2.10146484375
0.0599999999999999,2.12255859375
0.07,2.141015625
0.08,2.162109375
0.09,2.18056640625
0.1,2.20166015625
0.11,2.2201171875
0.12,2.2412109375
0.13,2.2623046875
0.14,2.278125
0.15,2.288671875
0.16,2.2939453125
0.17,2.29921875
0.18,2.29921875
0.19,2.29658203125
0.2,2.29130859375
0.21,2.2833984375
0.22,2.27548828125
0.23,2.26494140625
0.24,2.25439453125
0.25,2.24384765625
0.26,2.22802734375
0.27,2.21484375
0.28,2.20166015625
0.29,2.18583984375
0.3,2.17001953125
0.31,2.15419921875
0.32,2.1357421875
0.33,2.119921875
0.34,2.10146484375
0.35,2.08564453125
0.36,2.0671875
0.37,2.04873046875
0.38,2.03291015625
0.39,2.014453125
0.4,1.99599609375
0.41,1.9775390625
0.42,1.95908203125
0.43,1.940625
0.44,1.92216796875
0.45,1.9037109375
0.46,1.8826171875
0.47,1.86416015625
0.48,1.84306640625
0.49,1.824609375
0.5,1.803515625
0.51,1.78505859375
0.52,1.76396484375
0.53,1.74287109375
0.54,1.72177734375
0.55,1.70068359375
0.56,1.676953125
0.57,1.655859375
0.58,1.63212890625
0.59,1.60576171875
0.6,1.58203125
0.61,1.55302734375
0.62,1.5240234375
0.63,1.48974609375
0.64,1.45283203125
0.65,1.41328125
0.66,1.3658203125
0.67,1.233984375
0.68,1.065234375
0.69,0.9439453125
0.7,0.854296875
0.71,0.78046875
0.72,0.7224609375
0.73,0.67236328125
0.74,0.63017578125
0.75,0.5853515625
0.76,0.54052734375
0.77,0.49306640625
0.78,0.44560546875
0.79,0.3955078125
0.8,0.349091796875
0.81,0.29267578125
0.82,0.2423046875
0.83,0.18193359375
0.85,0.06591796875

